TTD: Text-Tag Self-Distillation Enhancing Image-Text Alignment in CLIP to Alleviate Single Tag Bias

We identify a critical bias in contemporary CLIP-based models, which we denote as single tag bias. This bias manifests as a disproportionate focus on a singular tag (word) while neglecting other pertinent tags, stemming from CLIP's text embeddings that prioritize one specific tag in image-text relationships. When deconstructing text into individual tags, only one tag tends to have high relevancy with CLIP's image embedding, leading to biased tag relevancy. In this paper, we introduce a novel two-step fine-tuning approach, Text-Tag Self-Distillation (TTD), to address this challenge. TTD first extracts image-relevant tags from text based on their similarity to the nearest pixels then employs a self-distillation strategy to align combined masks with the text-derived mask. This approach ensures the unbiased image-text alignment of the CLIP-based models using only image-text pairs without necessitating additional supervision. Our technique demonstrates model-agnostic improvements in multi-tag classification and segmentation tasks, surpassing competing methods that rely on external resources. The code is available at https://github.com/shjo-april/TTD.

==> sec/1_introduction.tex <==
\begin{figure}[!ht]
    \centering
    \includegraphics[width=\linewidth]{figures/fig1.pdf}
\caption{In existing image-text alignment research, \textit{single tag bias} is evident where the image and text embeddings tend to concentrate solely on a single tag. (a) \textbf{Single tag bias in image-text relationships}: When examining the similarity map between the image and text, it is evident that only a single tag inside the red box is activated, disregarding other elements mentioned in the text. (b) \textbf{Single tag bias in image-tag relationships}: Even when observing the similarity values between each tag in the text and the image, a high value is assigned only to the single tag, while other tags that describe the image exhibit similar values to insignificant tags. We used TCL~\cite{cha2023learning} for the analysis.}
\label{fig:single-tag-bias}
\end{figure}

\section{Introduction}
\label{sec:intro}
Research on fully supervised classification/segmentation is widely applied in the field of computer vision. Various weakly/semi-supervised and few-shot methods have emerged to reduce labeling costs, but there has been active research in image-text alignment following CLIP~\cite{radford2021learning}. Despite being trained solely on images and text (i.e., weak annotation), CLIP can be applied to downstream tasks that require stronger annotations, such as labels and masks. This study aims to improve CLIP performance using only weak information, which is in line with CLIP's original design intent.

 
As a major existing limitation to achieve this, we discover that CLIP-based models exhibit \textit{monofocus bias}, where they tend to overemphasize a particular context of image-text relationship. As observed in \cref{fig:single-tag-bias}(a), the similarity map between image and \textit{text} reveals activation only in the region related to a single tag/word (i.e., chameleon), while neglecting others (i.e., branch and green).  We termed this observed encoder output issue as \textit{single tag bias}, indicating a flaw in CLIP's pre-trained text encoder, which over-focuses on one tag, ignoring others.

Addressing this issue involves creating accurate foreground regions for every relevant tag, not just the biased one, to fine-tune the encoder to recognize their collective areas. It requires identifying all relevant tags in the text. However, testing each tag through CLIP's text encoder shows persistent \textit{single tag bias}, highlighting the challenge of extracting genuine tags solely with image-text pairs, as seen in \cref{fig:single-tag-bias}(b). This underlines the struggle of standard CLIP-based tag scoring due to the image encoder's reduction of pixel data to a singular tag focus, blocking the recognition of other image-relevant tags directly from text, illustrated by the pixels' overemphasis on one tag (i.e., jacuzzi in \cref{fig:overview}(a)), skewing the image's global (pooling-based) representation towards it. Even when scoring based on the proportion of pixels similar to each tag within the image as in segmentation, it still fails to lower scores for irrelevant tags, thus being unable to correctly extract meaningful tags from the text (see \cref{subsec:supp_tag}).


\begin{figure}[!t]
    \centering
    \includegraphics[width=\linewidth]{figures/fig2.pdf}
\caption{\textbf{High-level overview of our method.} (a) \textbf{Tag selection by pixel-tag scoring}: The pooled global image embedding predominantly reflects information about a single tag, which is ``jacuzzi'' in this example, due to the overactivation of a single tag in pixel embedding. (The colored similarity map in the figure shows the most relevant tag for each pixel.) By employing the maximum cosine similarity value between the tag and its most correlated pixel as a score, we minimize the impact of single tag bias observed in the image encoder. (b) \textbf{Text-tag self-distillation}: The similarity map between text and image demonstrates only a single tag, whereas it should represent all meaningful tags in the relationship between image and text. To alleviate the bias, we train the map between the image and text to align with the union of maps between the image and the pseudo tags obtained in (a), thus enhancing the image-text alignment. }
\label{fig:overview}
\end{figure}

To address this, we shift from standard global pooling to a new method focusing on the pixel index nearest to each tag candidate. This is based on the finding that pixels closely correlated with a specific tag more accurately pinpoint image segments, as shown in \cref{fig:overview}(a). By using the closest pixel's similarity to the tag as the measure for image-tag similarity, we counteract the bias, thus broadening the encoder's tag representation capacity.

We used pseudo tags from our scoring to remove unnecessary tag masks, creating valid foreground masks for all image-relevant tags. This led to a new self-distillation-based CLIP fine-tuning method, assuming optimal image-text relationships encompass all pseudo-tag contexts (Fig. \ref{fig:overview}(b)). We create a pseudo label, a union of the similarity maps between the image and all pseudo tags, making CLIP learn this as the real image-text map. This process enabled the model to recognize all related tag regions, not just one, improving CLIP's image-text alignment without additional data or annotations.

In summary, our contributions are as follows:
\begin{itemize}
    \item Identified bias in pre-trained CLIP models focusing on a single tag in image-text relationships.
    \item Proposed new scoring and self-distillation for training CLIP models with image-related tags extracted from text automatically.
    \item Achieved superior multi-tag classification and segmentation by enhancing image-text alignment using solely image-text pairs without external models. 
    \item Provided new tag/mask annotations related to text inputs for future open-vocabulary research. 
\end{itemize}

% \begin{itemize}
%     \item \sh{Identified bias in pre-trained CLIP models focusing on a single object/tag by text input.}
%     \item \sh{Proposed new scoring and self-distillation for training CLIP models with image-related tags extracted from text automatically.}
%     \item \sh{Achieved superior multi-tag classification and segmentation by enhancing pixel-tag alignment without external models.}
%     \item \sh{Provided new tag/mask annotations related to text inputs for future open-vocabulary research.}
% \end{itemize}


%This bias emerges from the objective of equalizing the single embeddings of image and text, so the model requires an objective with finer unit, word, that explicitly provide information about the relationship to mitigate such bias. 

%Simply, we extract words that well represent the image-text relationship from the text. The simple approach is to select words based on similarity between image and each word. 

% \begin{itemize}
% \item Identification of a single tag bias in CLIP-based models. Proposal of novel tag selection and self-distillation methods to address it. 
% \item Enhancement on the multi-tag selection in a model-agnostic manner and effectively resolved issues arising from the use of external NLP models.
% \item Consistent performance improvement in open-vocabulary semantic segmentation.
% \item Release of tag/mask annotations for future tag selection research and proposal of a new benchmark.
% \end{itemize}

%To resolve this, we deviate from the conventional global pooling-based representations, adopting a new method that utilizes the representation based on the index of the pixel closest to each tag candidate. Our observation informs this approach that pixels most correlated with a particular tag are better at accurately identifying the corresponding segments of an image as depicted in \cref{fig:overview}(a). By adopting the similarity measure between the tag and its most closely correlated pixel as the metric for the image-tag similarity, we effectively mitigate the bias issue, thereby significantly improving the encoder's capability to represent a broader array of tags accurately.
 
%Based on the pseudo tags selected by our scoring, we also suggest a text-tag distillation method that addresses single tag bias by text input. The ideal relationship between image and text should contain the context of all pseudo tags, not based only on a single tag. Thus, we generate an ideal similarity map between the image and text by unifying similarity maps between the image and the pseudo tags. Then, we distill this ideal map to the actual image-text map so that the model can learn to contain unbiased text context and thus enhance its alignment. \ks{Through fine-tuning, we enhanced the CLIP network's performance using only the given original training data (image and text-level), avoiding any extra supervision such as truth tags. This confirms CLIP's improved efficiency in multi-tag classification and segmentation among its downstream tasks, maintaining the initial setup of CLIP that uses text without awareness of the truth tag.}

%Our method is applicable to any model afflicted by single tag bias, as it enhances existing models through self-training using solely image and text data. It improves tag classification performance, tackling the issues associated with external NLP models. Furthermore, our method consistently enhances open-vocabulary semantic segmentation, signifying improved model alignment.


==> sec/2_related_works.tex <==
\section{Related works}
\label{sec:related_works}

CLIP~\cite{radford2021learning} stands out as the most prominent model for image-text alignment. It possesses a remarkable ability to comprehend various free-form texts, making it widely utilized in zero-shot/open-vocabulary scenarios. Consequently, various CLIP variants demonstrate comparable performance to models trained with task-specific annotations across many downstream tasks, such as classification and segmentation, even if they are trained with only image and text data. 

\input{tables/rel}
\begin{figure}[!t]
    \centering
    \includegraphics[width=\linewidth]{figures/fig3.pdf}
\caption{\textbf{A conceptual comparison between previous approaches and ours.} (a) Image-text alignment models, while useful for various open-vocabulary tasks, suffer from single tag bias. To alleviate this bias, extracting tags that reflect the image-text relationship from the text for training is crucial. (b) However, existing research often relies on external NLP models to extract tags without considering images, leading to issues: 1) Extracting image-irrelevant tags. 2) Overlooking image-relevant tags. (c) In contrast, we propose a tag selection method using only pixel information from images, eliminating the need for reliance on external models.}
\label{fig:alignment}
\end{figure}

\subsection{CLIP Variants with Pixel-Text Alignment}
CLIP faces challenges in downstream tasks requiring localization (e.g., segmentation and detection). Consequently, recent models~\cite{cha2023learning, yi2023simple, zhou2022extract, liu2022open, ranasinghe2023perceptual} have emerged that learn pixel-text alignment solely from image-text data without additional annotations. 
TCL~\cite{cha2023learning} generates a text-grounded mask that represents the relationship between an image and corresponding text, then aligns the text-grounded image and the text. SimSeg~\cite{yi2023simple} aims to align a sparse portion of the image and the text that only contains critical information. While these studies showcase impressive performance, they still exhibit single tag bias in image-text relationships as shown in \cref{tab:captioniou} as they implicitly learn alignment from the text. In contrast, our method extracts meaningful tags from the text and uses them for learning to alleviate the bias. 

\subsection{CLIP Variants with Tag Selection}  

\subsubsection{Utilization of External NLP models} 
Recent studies~\cite{liang2023open, mukhoti2023open, xu2022groupvit, xu2023learning, liu2023tagalign} have focused on extracting tags from text for learning, relying on external NLP models (\cref{fig:alignment}(b)). While some studies utilize NLP parsers~\cite{loper2002nltk, spacy2, akbik2019flair} to extract nouns, others leverage Large Language Models (LLM) like Vicuna~\cite{chiang2023vicuna}. However, these tag selection techniques entirely disregard image information, resulting in two issues as shown in \cref{fig:qual_tag}: 1) Extracting image-irrelevant tags. 2) Overlooking image-relevant tags, particularly non-nouns. However, our method is free from such issues since we only utilize the image and text for tag selection. 

\subsubsection{Additional Filtering using Image Information} Some models~\cite{xing2024rewrite, conti2024vocabulary} additionally consider the image to score tags. However, they utilize globally pooled image representation, suffering from single tag bias (\cref{fig:single-tag-bias}(b)). CoCu~\cite{xing2024rewrite} additionally introduces scoring based on retrieved image relevancy, but this depends on the images retrieved, where tag-relevant images lead to a low score and vice versa, and also requires high computational cost (see \cref{subsec:supp_tag}). Also, both models rely on external NLP models and fail to address the omission of image-relevant tags.

Our proposed tag selection method scores tags based on the relationship between a tag and its most correlated pixel without employing external NLP models or data. This method mitigates single tag bias of image embedding and problems of external NLP models as shown in \cref{tab:ovc_tagacc}. Then, we present a text-tag self-distillation method to enhance pixel-tag alignment to address single tag bias in image-text relationships. As this approach uses only image and text data without additional annotations, it can be applied in a model-agnostic manner.

==> sec/3_method.tex <==
\begin{figure}[!t]
    \centering
    \begin{subfigure}{\textwidth}
        \includegraphics[width=\textwidth]{figures/fig4_1.pdf}
        \caption{Tag Selection by Pixel-Tag Scoring}
        \label{fig:tagging}
    \end{subfigure}
    \hfill
    \begin{subfigure}{\textwidth}
        \centering
        \includegraphics[width=0.9\textwidth]{figures/fig4_2.pdf}
        \caption{Method Overview}
        \label{fig:overview_all}
    \end{subfigure}            
\caption{\textbf{Overall framework of our method.} (a) \textbf{Tag selection by pixel-tag scoring}: Utilizing the similarity with the most correlated pixel as scoring, we identify a significant gap between tags related to the image and irrelevant ones. This gap guides us in selecting tags with the largest score gap as the threshold.
(b) \textbf{Method overview}: Our fine-tuning approach begins by obtaining pseudo tags through our tag selection process, which are then used to create an ideal heatmap representing the image-text relationship. We address single tag bias by distilling information between the ideal and actual heatmaps. Additionally, we integrate an auxiliary loss to learn the pixel-tag relationship. Throughout this process, both the image and text encoders are trained.
}
\label{fig:method-overview}
\end{figure}

\section{Method}
\label{sec:method}

Our fine-tuning method that alleviates single tag bias consists of two stages: Tag selection by pixel-tag scoring (\cref{subsec:tagging}) and Text-tag self-distillation (\cref{subsec:fine-tune}). The overall framework is illustrated in \cref{fig:method-overview}.

\subsection{Tag Selection by Pixel-Tag Scoring}
\label{subsec:tagging}

Given an image $I$ of size $H\times W$ and corresponding text $T$ composed of tags $ \mathcal{T}=\{t_1 \cdots t_n\}$, our objective is to extract tags, $\mathcal{T}_{gt} \subset \mathcal{T}$ that accurately represent the image-text relationship. (e.g. for the first image in \cref{fig:qual_tag}, $\mathcal{T}_{gt}=\{t_1, t_2, t_3, t_6, t_7\}$.) Importantly, our approach relies solely on the image $I$ and the text $T$, without any external datasets or models.

Let $\mathcal{E}_V, \mathcal{E}_T$ denote the image and text encoders, respectively, which provide pixel embeddings and global text embeddings: $\mathcal{E}_V(I)\in \mathbb{R}^{H\times W\times C},\mathcal{E}_T(T)\in \mathbb{R}^C$ where $C$ is the embedding dimension size of the encoder output and $H, W$ are height and width of the image. The global image embedding can be obtained by globally average pooling the pixel embedding: $\mathrm{gap}(\mathcal{E}_V(I)) \in \mathbb{R}^C$. 

A simple approach involves using the similarity between the image and a tag as a score:
\begin{equation} \label{eq:s_image}
    s_{\mathrm{image}}(t_i) := \mathrm{sim}(\mathrm{gap}(\mathcal{E}_V(I)), \mathcal{E}_T(t_i)),
\end{equation}
where $\mathrm{sim}$ denotes similarity metric, and cosine similarity is used in our case. However, this scoring method is affected by single tag bias, as depicted in \cref{fig:single-tag-bias}(b). This bias originates from the tendency of most pixels to be biased towards a specific tag, as shown in \cref{fig:overview}(a), thereby overlooking other relevant tags.

To mitigate this issue, we propose a novel scoring approach that leverages the pixel embedding most correlated with a tag rather than relying on a global image embedding:
\begin{equation} \label{eq:s_pixel}
    s_{\mathrm{pixel}}^{\mathrm{ours}}(t_i) := \max_{1\leq h \leq H, 1 \leq w \leq W} \mathrm{sim}(\mathcal{E}_V(I)_{hw}, \mathcal{E}_T(t_i)).
\end{equation}
This approach ensures more accurate consideration of objects within the image since each pixel corresponds to its most similar object. Utilizing pixel embeddings from the stage before pooling to compute similarity scores increases computational overhead compared to a simple approach. However, it can be reused because the computed similarity map is used for distillation in the subsequent step (\cref{subsec:fine-tune}).

Subsequently, we notice a substantial score gap between tags associated with the image and those not. As illustrated in \cref{fig:method-overview}(a), we arrange all tags according to $ s_{\mathrm{pixel}}^{\mathrm{ours}}$ and compute the score difference between consecutive tags. We observed the significantly large score difference between meaningful tags and others at the boundary. Leveraging this observation, we extract pseudo tags with high scores using the largest score gap as the boundary: $\mathcal{T}_{pred} \subset \mathcal{T}$. 

Our pixel-tag scoring ($s_{\mathrm{pixel}}^{\mathrm{ours}}$) is derived through a straightforward calculation similar to the simple approach ($s_{\mathrm{image}}$). However, it showcases outstanding tag selection performance and effectively addresses issues encountered by methods employing external NLP models as seen in \cref{tab:ovc_tagacc}. Furthermore, unlike $s_{\mathrm{image}}$, which relies on heuristic methods like selecting the top-$k$ tags or setting a constant threshold due to insignificant score differences beyond the major tag, our tag selection method automatically identifies appropriate tags.


\subsection{Text-Tag Self-Distillation}
\label{subsec:fine-tune}
In this section, we introduce a self-distillation technique designed to mitigate single tag bias arising from text embedding (\cref{fig:single-tag-bias}(a)). The pseudo tags $\mathcal{T}_{pred}$ obtained from our tag selection method (\cref{subsec:tagging}) encapsulate the relationship between the image and the text, enabling the transfer of knowledge from pseudo tags to the text. Specifically, we ensure alignment between the union of similarity maps of pseudo tags and the image with that of the text and image:
\begin{equation} \label{eq:simmap}
    \mathrm{sim}(x) := \mathrm{sim}(\mathcal{E}_V(I), \mathcal{E}_T(x)) \in \mathbb{R}^{H\times W},
\end{equation}
\begin{equation} \label{eq:L_distill}
    \mathcal{L}_{distill} = ||\mathrm{sim}(T) - \bigcup_{t_i\in \mathcal{T}_{pred}} \mathrm{norm}(\mathrm{sim}(t_i))||^2_2,
\end{equation}
where $\mathrm{sim}(x)$ is an abbreviation of the similarity map between the image $I$ and a text $x$, $\bigcup$ is the pixel-wise (element-wise) maximum operation, and $\mathrm{norm}$ is min-max normalization. Here, we apply a stop-gradient operation on the union similarity map to propagate the gradients only through the text-based one. 

Additionally, we introduce an auxiliary loss function to reinforce the correlation between tags and the image. Tags that are not selected are deemed irrelevant to the image; thus, we drive their similarity map toward zero. Conversely, selected tags are trained to align with the discrete map to disregard unrelated image parts:
\begin{equation} 
    \mathcal{L}_{tag} = \sum_{t_i \in \mathcal{T}} D(t_i) \ \mathrm{, where} \ D(t_i) = \begin{cases}
        ||\mathrm{sim}(t_i) - \mathrm{norm}(\mathrm{sim}(t_i))||^2_2 &\mathrm{if} \ t_i \in \mathcal{T}_{pred}\\
        ||\mathrm{sim}(t_i)||^2_2 &\mathrm{otherwise}
    \end{cases}.
    \label{eq:L_tag}
\end{equation}
Similar to text-tag distillation loss, we apply a stop-gradient operation on the normalized masks.

Our final fine-tuning loss function is defined as follows:
\begin{equation} \label{eq:L_final}
    \mathcal{L} = \mathcal{L}_{distill} + \mathcal{L}_{tag}.
\end{equation}

Some may question whether it is more effective to view segment-level relationships using external models like SAM~\cite{kirillov2023segment} rather than examining pixel-level relationships. However, our method is unrestricted and versatile since we self-train the model utilizing only image and text information without additional supervision, such as ground-truth tag annotation or external models. We also provide supplementary experiments on advanced techniques utilizing external models in \cref{subsec:supp_sam}.

==> sec/4_experiments.tex <==
\definecolor{md}{rgb}{1.0,0.2,0.2}
\definecolor{ud}{rgb}{0.2,0.6,1.0}

\section{Experiments}
\label{sec:exp}

\subsubsection{Datasets and Implementation detail}
In all experiments, we trained our model solely with image-text pairs without utilizing additional annotations like truth tag information for the text. We demonstrated its flexibility by evaluating its performance on two distinct public models~\cite{zhou2022extract, cha2023learning}. Furthermore, to cut computational costs, we utilized the LoRA~\cite{hu2021lora} technique for all our training processes. We used the CC3M and CC12M datasets~\cite{sharma2018conceptual, changpinyo2021conceptual} for training, applying an additional sample filtering strategy to reduce the use of largely uncorrelated image-text pairs. 

To evaluate the performance of our tag selection method, we manually collected truth tag information for all image-text pairs of CC3M validation set~\cite{sharma2018conceptual}. Also, to see how much the single tag bias has eased, we generated the tag's corresponding mask data for 680 image-text pairs. This was necessary because, to our knowledge, there is no existing dataset that provides a complete match of all truth tags and their corresponding masks with the text. We will make this information available through code release. Details are in \cref{sec:supp_dataset}. 

Additionally, for assessing our method's effectiveness in open-vocabulary semantic segmentation using tag inputs, we use six established benchmarks: PASCAL VOC (VOC)~\cite{everingham2010pascal}, PASCAL Context (Context)~\cite{mottaghi2014role}, COCO-Stuff (Stuff), COCO-Object (Object)~\cite{caesar2018coco}, Cityscapes (City)~\cite{cordts2016cityscapes}, and ADE20k (ADE)~\cite{zhou2019semantic}. Further evaluations on segmentation performance with referring datasets, alongside conventional open-vocabulary classification tasks, and specifics of these assessments are detailed in \cref{subsec:supp_impl} and \ref{sec:supp_add_exps}.


\subsubsection{Evaluation metrics}
For evaluating tag selection, we use metrics like precision, recall, accuracy, F1 score, and mean Average Precision (mAP) as established in existing studies~\cite{he2023open, li2023patchct}. Precision measures the fraction of accurately identified positive tags among all predicted as positive, and recall quantifies the fraction of accurately identified positive tags out of all true positive tags. Notably, since there is no predetermined label set, we adopt sample-wise mAP~\cite{kobayashi2023two} over the standard class-wise mAP.

To evaluate segmentation performance, we use mean Intersection over Union (mIoU). For our proposed benchmark, considering the assessment of a model's ability to capture the relationship between captions and images, we refer to this mIoU as CaptionIoU. Furthermore, given our binary mask annotation, we also report the mean false positive rate (mFPR) and mean false negative rate (mFNR) to provide a comprehensive assessment of segmentation quality. 


\subsection{Main Results}
\label{subsec:exp_main}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.9\linewidth]{figures/fig5.pdf}
\caption{\textbf{Qualitative results of tag selection.} Tag selection using external models~\cite{loper2002nltk, chiang2023vicuna, bai2023qwen} suffers from two problems because they do not consider image information. {\textbf{1) Extracting image-irrelevant tags (\textcolor{md}{red}):} Select tags that do not correlate with the corresponding image content.} {\textbf{2) Overlooking image-relevant tags (\textcolor{ud}{blue}):} Cannot select tags related to the image, particularly non-nouns in the case of NLTK.}}
\label{fig:qual_tag}
\end{figure}
% misdetected tags 가 우리보다 못하는 예시도 필요할 것 같음. 
\input{tables/exp_cls_tagacc}

\subsubsection{Multi-Tag Selection}
\label{subsubsec:exp_tagacc}
We assess the performance of our pixel-tag scoring-based method (Sec. \ref{subsec:tagging}) in the multi-tag selection task (i.e., the performance to identify all image-related tags given only the text without prior knowledge of the tags such as pre-defined label set). This evaluation is conducted in comparison to methods that use NLP models~\cite{loper2002nltk, chiang2023vicuna, bai2023qwen} and other basic scoring techniques. For scoring, we utilize image and text encoders from TCL~\cite{cha2023learning}, setting the threshold for other scoring approaches at 0.5.

%We evaluate the tag selection performance (i.e., identifying all image-related truth tags without knowledge of them and only the text are given) of our pixel-tag scoring-based method (\cref{subsec:tagging}) against approaches utilizing NLP models~\cite{loper2002nltk, chiang2023vicuna, bai2023qwen} and various simple scoring methods. For scoring, we employ image and text encoders from TCL~\cite{cha2023learning}, while the threshold for other scoring methods defaults to $0.5$.

As depicted in \cref{fig:qual_tag}, tag selection with external NLP models encounters two main issues: identifying tags not pertinent to the image and missing relevant tags due to ignoring visual information. As seen in the last example, NLTK selects irrelevant tags (e.g., `/') due to the overfit on pre-trained sentence structures. Nonetheless, our method largely extracts tags relevant to the image, addressing significant issues in conventional NLP models, especially identifying tags relevant to the image.  


This superiority is further evident in \cref{tab:ovc_tagacc}. Higher precision indicates better filtering of image-irrelevant tags, while higher recall denotes improved extraction of image-relevant tags. As shown in \cref{tab:ovc_tagacc}(a), NLTK, the most widely used NLP parser for tag selection, exhibits high recall but at the expense of low precision, as it extracts all nouns without considering image information. Large Language Models (LLMs) show inferior performance compared to ours due to hallucination issues and lack of image consideration. In contrast, our method outperforms NLP models in both F1 score and accuracy with a significant margin, showing even better performance after fine-tuning. This indicates that our method effectively addresses the limitations of NLP models.

\cref{tab:ovc_tagacc}(b) presents the tag selection performance with different scoring methods. Following \cite{conti2024vocabulary}, we define a score that measures the similarity between the text and tag in addition to image-tag scoring ($s_{\mathrm{image}}$):
\begin{equation} \label{eq:s_text}
    s_{\mathrm{text}}(t_i) := \mathrm{sim}(\mathcal{E}_T(T), \mathcal{E}_T(t_i)).
\end{equation}

% Moreover, \cite{li2023clip} adopted a scoring strategy by extracting tag embedding from token embeddings, not directly inputting tags to the text encoder. Specifically, when the text $T$ is provided to the text encoder, it undergoes tokenization, and embeddings for each token are generated. Here, the tag embedding is derived by averaging the embeddings of all tokens constituting the tag. For example, the embedding of `neckline' is the average of the embeddings of `neck' and `line'. Typically, a tag consists of a single token most of the time. The final score is calculated as the similarity between generated tag embedding and a global image embedding:
% % Moreover, \cite{li2023clip} adopted a scoring strategy by extracting tag embedding from text embedding, not directly inputting tags to the text encoder:
% \begin{equation} \label{eq:s_token}
%     s_{\mathrm{token}}(t_i) := \mathrm{sim}(\mathcal{E}_T(T), \mathcal{E}_T'(t_i)),
% \end{equation}
% where $\mathcal{E}_T'(t_i)$ is an abbreviation of an average of embeddings of tokens that construct the tag $t_i$. 
% % tag embedding generated from text embedding. 



%While image-tag scoring ($s_{\mathrm{image}}$) displays high precision, it suffers from very low recall due to single-tag bias by tag input, resulting in the selection of only one tag most of the time. The text-tag scoring ($s_{\mathrm{text}}$) exhibits similar behavior, as does their combination. The image-token scoring ($s_{\mathrm{token}}$) performs poorly, indicating that the token embeddings of the entire text do not interpret each tag well. However, our method shows significant improvement, addressing single-tag bias by tag input. We also discuss sensitivity to thresholds and other scoring methods utilizing external data in addition to an image-text pair in Appendix.

% The performance of the scoring using token embeddings ($s_{\mathrm{token}}$) is not satisfactory. This indicates that each token embedding fails to adequately represent the token, suggesting that when utilizing the output of the text encoder, it is preferable to use text embeddings, rather than token embeddings. 
While image-tag scoring (\(s_{\mathrm{image}}\)) demonstrates high precision, it experiences very low recall due to the single tag bias, often leading to the selection of only one tag so if misses other image-related tags. Similarly, text-tag scoring (\(s_{\mathrm{text}}\)) and their combination show comparable issues. However, our approach significantly mitigates the single tag bias, showing high recall. Also, it exhibits high accuracy and mAP, which indicates the effectiveness of our scoring method. We further examine sensitivity to different thresholds and alternative scoring techniques that incorporate external data beyond the image-text pair in \cref{subsec:supp_tag}.

\subsubsection{Text-level Semantic Segmentation}
\label{subsubsec:exp_captioniou}
In this task, we evaluate text-level segmentation performance, where the text encoder of CLIP processes text input using existing CLIP-based models~\cite{cha2023learning, zhou2022extract} and followed by the application of our fine-tuning method, TTD. Specifically, this task evaluates whether the model accurately understands the relationship between the image and the given text. As depicted in \cref{fig:qual_ciou}, traditional models show a single tag bias, mainly capturing the spatial region of only one tag. TCL often generates masks that extend beyond the relevant context. Yet, after fine-tuning with our method, the single tag bias reduces, and the fine-tuned models accurately activate all regions associated with image-related tags in the respective text.
% In contrast, our method alleviates this bias, resulting in masks that effectively represent the provided text.

The effectiveness of TTD is further illustrated in \cref{tab:captioniou}, where its integration enhances the models' comprehension of the text-image relationship, leading to improved CaptionIoU scores (i.e., +7.2\% on average). Notably, MaskCLIP exhibits a significant decrease in the mFNR score (i.e., 0.169) post-fine-tuning, indicating its improved understanding beyond a single tag. Additionally, TCL demonstrates a noteworthy decrease in mFPR. It means that after fine-tuning, the model can exclude portions unrelated to the text, indicating that our fine-tuning method enhances model alignment as well.

\begin{figure}[!t]
    \centering
    \includegraphics[width=0.95\linewidth]{figures/fig6.pdf}
\caption{\textbf{Qualitative results on text-level segmentation.}}
\label{fig:qual_ciou}
\end{figure}
\input{tables/exp_seg_text}


\subsection{Results on Open-Vocabulary Semantic Segmentation}
\label{subsec:exp_ovs}

In the previous task, we evaluated the classification and segmentation performance of TTD-trained CLIP using text input, measuring how well the model understands the relationship between the image and the text. Subsequently, we conducted experiments on standard open-vocabulary semantic segmentation where the text encoder was provided with tag input. Note that our TTD training did not utilize actual tag annotation from the text. In \cref{fig:qual_ovs}, we display segmentation results with and without TTD. Our approach effectively detects the presence of objects in the image, unlike conventional models that identify objects not actually present in the image.

\cref{tab:ovs} contrasts the tag-level segmentation performance of studies employing only image-text pairs without additional annotations or external models akin to ours for fair comparison. For this reason, models~\cite{liang2023open, ding2022decoupling, luo2023segclip, guo2023mvp} that utilize additional annotations or external models (e.g. mask proposal networks) are also excluded. Additionally, we compared models that utilize NLP-based models($\mathcal{L}$ in the table) for tag extraction. Implementing our fine-tuning technique results in an average increase in mIoUs of 8.5\% for MaskCLIP and 3.5\% for TCL. Furthermore, TCL enhanced with our method outperforms existing models on benchmarks such as Pascal VOC, Pascal Context, and COCO-Object. This indicates that our approach successfully augments model alignment in addition to alleviating single tag bias.

At this point, TagAlign~\cite{liu2023tagalign} achieved better performance on datasets that have at least 150 classes such as COCO-Stuff/ADE20K than our model. The reason for this is that TagAlign utilized multiple text information for a single image, whereas we opted for simplicity by using only a single text corresponding to each image. Therefore, the performance difference arises from the relatively insufficient positive/negative tag information in our method, indicating the potential value in further improving our fine-tuning method.


\begin{figure}[!t]
    \centering
    \includegraphics[width=0.8\linewidth]{figures/fig7.pdf}
\caption{\textbf{Qualitative results on tag-level segmentation.}}
\label{fig:qual_ovs}
\end{figure}
\input{tables/exp_ovs}


\subsection{Ablation}
\label{subsec:exp_ab}
\input{tables/exp_ab}

In this section, we conducted ablation experiments to evaluate the impact of the techniques employed in our fine-tuning method. The assessment was performed using TCL~\cite{cha2023learning} on our text-level, and Pascal VOC~\cite{everingham2010pascal} for tag-level segmentation.

\subsubsection{Effect of Fine-tuning Losses} Our method incorporates two loss terms, $\mathcal{L}_{distill}$ and $\mathcal{L}_{tag}$, for fine-tuning. $\mathcal{L}_{distill}$ aims to mitigate single tag bias, while $\mathcal{L}_{tag}$ aims to enhance the pixel-tag correlation. When solely utilizing $\mathcal{L}_{tag}$, there was a marginal performance enhancement observed during the min-max normalization process for each mask, as depicted in \cref{tab:ab}(a). However, the inclusion of $\mathcal{L}_{distill}$ significantly alleviates single tag bias, leading to an improvement in both CaptionIoU and mIoU (i.e., +3.2\% and +5.8\%, respectively). The best performance is achieved when both losses are combined, learning each tag mask and union mask simultaneously.

\subsubsection{Effect of Tag Selection Method}
\label{subsubsec:exp_ab_tagging}
In our approach, tag selection is conducted via pixel-tag scoring (\cref{eq:s_pixel}) to extract pseudo tags representing the image-text relationship. Alternatively, we examine NLTK and simple image-tag scoring (\cref{eq:s_image}) for tag selection, as shown in \cref{tab:ab}(b). When employing NLTK to extract nouns from texts, due to the aforementioned issues (extraction of image-irrelevant tags and omission of image-relevant tags), the model struggles to generate the ideal text-image similarity map (i.e., the union of pseudo-tag driven maps). Consequently, the generated union map may include the activation of unrelated tags or omit activations necessary for the image-tag relationship, resulting in minor improvement. On the other hand, using image-tag scoring tends to extract a single tag, exacerbating single tag bias and resulting in a decline in both CaptionIoU and mIoU. In contrast, our tag selection method exhibits significantly enhanced performance in both tasks, indicating that the pseudo tags extracted using our method effectively capture the relationship between image and text.

==> sec/5_conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}
Our research addresses the misalignment between images and text inherent in existing CLIP-based models. Specifically, we present a fine-tuning technique that resolves the issue where image and text representations are overly focused on a single tag, thereby enhancing both image segmentation and multi-tag classification within the text. This was achieved using only image and text pairs, without additional annotations. The key outcome of addressing the single tag bias is enabling CLIP to correctly identify all truth tags related to the image within the text, akin to how class activation map studies provide pixel-level class information without direct input to the network. Our TTD training method, which does not employ external modules for tag extraction, ensures that the predicted tags by the fine-tuned model have direct relevance to the image. This feature can effectively address the hallucination issue seen in conventional tag generation models, where natural language processing-based models might generate tags unrelated to the target image. Hence, our approach is valuable as it offers a solution to the hallucination problem, suggesting significant potential for various applications.
%We present a two-stage fine-tuning method designed to mitigate the single tag bias prevalent in existing CLIP-based models. Our approach addresses this bias through tag selection using pixel-tag scoring and text-tag distillation techniques. Firstly, our novel tag selection method effectively extracts meaningful tags from text, relying solely on image and text data. This approach not only mitigates single tag bias by tag input but also resolves issues associated with the use of external NLP models. Secondly, through text-tag distillation, we further mitigate single tag bias by text input. Importantly, our method operates in a model-agnostic manner, making it applicable to any model affected by single tag bias. By leveraging only image and text data, our approach offers a practical and effective solution for improving the alignment of CLIP-based models in various applications.

==> tables/exp_cls_single.tex <==
% \definecolor{Gray}{gray}{0.85}
\definecolor{pink}{rgb}{0.96,0.82,0.82}

% \setlength{\tabcolsep}{1.5pt}
\begin{table}[tb]
  \caption{Open-Vocabulary Single-Label Classification. We used ViT-B/16 for backbone for all methods. Sup., supervision; FS, few-shot; ZS, zero-shot; D, using additional datasets; C101, Caltech101; ESAT, EuroSAT; Airc., FGVC-Aircraft; Flwr, Flowers-102; Food, Food-101; Pets, Oxford Pets; Cars, Stanford Cars; SUN, SUN397; UCF, UCF101; ImageNet1k, IN1k.}
  \label{tab:ovc_single}
  \centering
  \resizebox{0.85\textwidth}{!}{
  \begin{tabular}{@{}lccccccccccccc@{}}
    \toprule
    Method & Sup. & C101 & DTD & ESAT & Airc. & Flwr & Food & Pets & SUN & Cars & UCF & IN1k & Avg. \\
    \midrule
    \midrule
    CoOp~\cite{zhou2022learning}    & FS &  &  &  &  &  &  &  &  &  &  &  &  \\
    PLOT~\cite{chen2022prompt}    & FS &  &  &  &  &  &  &  &  &  &  &  &  \\
    CaSED~\cite{conti2024vocabulary}    & ZS+D &  &  &  &  &  &  &  &  &  &  &  &  \\
    \midrule
    CLIP~\cite{radford2021learning}    & ZS &  &  &  &  &  &  &  &  &  &  &  &  \\
    \rowcolor{pink}
    + Ours          & ZS &  &  &  &  &  &  &  &  &  &  &  &  \\
    SimSeg~\cite{yi2023simple}    & ZS &  &  &  &  &  &  &  &  &  &  &  &  \\
    \rowcolor{pink}
    + Ours          & ZS &  &  &  &  &  &  &  &  &  &  &  &  \\
    TCL~\cite{cha2023learning}    & ZS & 86.0 & 40.5 & 37.9 & 7.5  & 32.7 & 53.3 & 57.0 & 35.5 & 25.3 & 48.6 & 43.3 &  \\
    \rowcolor{pink}
    + Ours                        & ZS & 88.4 & 41.9 & 39.7 & 12.4 & 34.3 & 37.7 & 62.2 & 40.1 & 28.1 & 47.8 & 53.5 &  \\
  \bottomrule
  \end{tabular}
  }
\end{table}

==> tables/exp_supp_tag_sensi.tex <==
\definecolor{pink}{rgb}{0.96,0.82,0.82}

\setlength{\tabcolsep}{1.5pt}
\begin{table}[!tb]
  \caption{\textbf{Sensitivity of scoring methods based on threshold}. 
  % We utilize image and text encoders from TCL~\cite{cha2023learning} for scoring.
  }
  \label{tab:supp_tagacc_thrd}
  \centering
  \resizebox{0.5\textwidth}{!}{
  \begin{tabular}{@{}lccccc@{}}
    \toprule
    Scoring & P & R & F1 & Acc & mAP\\
    \midrule
    \midrule
    $s_{\mathrm{image}}$ (\cref{eq:s_image})        & 92.5 & 28.6 & 43.7 & 79.5 & 83.2 \\ 
    \midrule
    $s_{\mathrm{pixel}}^{\mathrm{ours}}$ (\cref{eq:s_pixel})        & 82.9 & 74.5 & 78.5 & 88.6 & 90.3 \\
    + TTD (Ours)        & 88.3 & 78.0 & 82.8 & 91.0 & 93.7 \\
  \bottomrule
  \end{tabular}
  }
\end{table}
